RuleFlow : Generating Reusable Program Optimizations with LLMs

Optimizing Pandas programs is a challenging problem. Existing systems and compiler-based approaches offer reliability but are either heavyweight or support only a limited set of optimizations. Conversely, using LLMs in a per-program optimization methodology can synthesize nontrivial optimizations, but is unreliable, expensive, and offers a low yield. In this work, we introduce a hybrid approach that works in a 3-stage manner that decouples discovery from deployment and connects them via a novel bridge. First, it discovers per-program optimizations (discovery). Second, they are converted into generalised rewrite rules (bridge). Finally, these rules are incorporated into a compiler that can automatically apply them wherever applicable, eliminating repeated reliance on LLMs (deployment). We demonstrate that RuleFlow is the new state-of-the-art (SOTA) Pandas optimization framework on PandasBench, a challenging Pandas benchmark consisting of Python notebooks. Across these notebooks, we achieve a speedup of up to 4.3x over Dias, the previous compiler-based SOTA, and 1914.9x over Modin, the previous systems-based SOTA. Our code is available at https://github.com/ADAPT-uiuc/RuleFlow.

==> sections/background.tex <==
\section{Background}
\label{sec:background}



==> sections/tables/error_analysis.tex <==
{\footnotesize
\begin{table*}[t]
\caption{Error Categories}
% \sffamily
% \setlength{\arrayrulewidth}{1.05pt} 
\begin{tabular}{@{}|p{0.10\textwidth}|p{0.20\textwidth}|p{0.20\textwidth}|p{0.25\textwidth}|p{0.10\textwidth}|@{}}
\hline
%Row 1
\rowcolor{lightgray!15}
Category & \centering LHS & \centering RHS & \centering Preconditions & Impacted Notebooks\arraybackslash \\
\hline
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
% % \vspace{0pt}
\scriptsize
Reference \\
Errors
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{df}|} = @{|\highlightast{Name}|: |\highlightvar{df}|}.drop(@{|\highlightast{expr}|: |\highlightvar{e1}|}, axis=1)
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
for col in @{|\highlightvar{e1}|}:
    del @{|\highlightvar{df}|}[col]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
[is(@{|\highlightvar{df}|}, pd.DataFrame),
all(is(col, str) for col in @{|\highlightvar{e1}|}),
all(col in @{|\highlightvar{df}|}.columns for col in @{|\highlightvar{e1}|})]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
% \vspace{0pt}
$1/102$
\end{minipage}
\\
\hline
%Row 2
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\scriptsize
Semantic \\
Divergence due \\
to Null Values \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{n1}|} = @{|\highlightast{expr}|: |\highlightvar{e1}|}.max()
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
@{|\highlightvar{n1}|} = np.max(@{|\highlightvar{e1}|}.to_numpy())
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
[np == numpy,
type(@{|\highlightvar{e1}|}) == pandas.Series]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
% \vspace{0pt}
$?$
\end{minipage}
\\
\hline
%Row 3
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\scriptsize
Semantic \\
Hallucinations \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{n2}|} = @{|\highlightast{Name}|: |\highlightvar{n1}|}.isnull().sum()
@{|\highlightast{Name}|: |\highlightvar{n3}|} = @{|\highlightvar{n2}|}[@{|\highlightast{Slice}|: |\highlightvar{s1}|}]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
@{|\highlightvar{n3}|} = @{|\highlightvar{n1}|}.iloc[:, :10].isnull().sum()
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15, escapeinside=||]{python}
[type(@{|\highlightvar{n1}|}) == pandas.DataFrame,
type(@{|\highlightvar{n2}|}) == pandas.Series,
@{|\highlightvar{n2}|}.index.equals(@{|\highlightvar{n1}|}.columns)]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
% \vspace{0pt}
$?$
\end{minipage}
\\
\hline
%Row 4
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\scriptsize
Syntactical \\
Errors \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
% \vspace{0pt}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
% \vspace{0pt}
$?$
\end{minipage}
\\
\hline
\end{tabular}
% \vspace{2pt}
\label{tbl:error_rules}
\end{table*}
}


==> sections/tables/plebian.tex <==
{
\footnotesize
\begin{table*}[t]
\caption{Plebian Categories}
% \sffamily
% \setlength{\arrayrulewidth}{1.5pt} 
\begin{tabular}
{@{}|p{0.10\textwidth}|p{0.2\textwidth}|p{0.2\textwidth}|p{0.26\textwidth}|p{0.04\textwidth}|p{0.04\textwidth}|@{}}
\hline
%Row 1
\rowcolor{lightgray!15}
Category & \centering LHS & \centering RHS & \centering Preconditions & \centering Spd & \centering Freq\arraybackslash \\
\hline
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\scriptsize
Expensive \\
Preconditions \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{n1}|}= @{|\highlightast{Name}|: |\highlightvar{n2}|}.sample(@{|\highlightast{Const(int)}|: |\highlightvar{c1}|})
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15,escapeinside=||]{python}
@{|\highlightvar{n1}|}= @{|\highlightvar{n2}|}.loc[np.random.choice(@{|\highlightvar{n2}|}.index, size=@{|\highlightvar{c1}|}, replace=False)]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
[is(@{|\highlightvar{n2}|}, (pd.DataFrame, pd.Series)), @{|\highlightvar{c1}|} <= len(@{|\highlightvar{n2}|}), 
@{|\highlightvar{c1}|} >= 0, @{|\highlightvar{n2}|}.index.is_unique]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$0.64\times$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
\\
\hline
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\scriptsize
Datasize \\
Discrepensy \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{n2}|}[ @{|\highlightast{expr}|: |\highlightvar{e1}|} ][ @{|\highlightast{Const(str)}|: |\highlightvar{c1}|} ].unique()
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15,escapeinside=||]{python}
@{|\highlightvar{n1}|}= np.unique(@{|\highlightvar{n2}|}.loc[@{|\highlightvar{e1}|}, @{|\highlightvar{c1}|}].values)
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
[is(@{|\highlightvar{n2}|}, pd.DataFrame),@{|\highlightvar{c1}|} in @{|\highlightvar{n2}|}.columsns,
is(@{|\highlightvar{e1}|}, (np.ndarray, pd.Series, pd.Index, list)) or
hasattr(@{|\highlightvar{e1}|}, '__array__')]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?\times$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
\\
\hline
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\scriptsize
Insufficient \\
Generalization \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{n1}|}= @{|\highlightast{Name}|: |\highlightvar{n2}|}.groupby(@{|\highlightast{Const(str)}|: |\highlightvar{c1}|})[@{|\highlightast{Const(str)}|: |\highlightvar{c2}|}].count().plot(kind=@{|\highlightast{Const(str)}|: |\highlightvar{c3}|})
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15,escapeinside=||]{python}
@{|\highlightvar{n1}|}= @{|\highlightvar{n2}|}[@{|\highlightvar{c1}|}].value_counts().plot(kind=@{|\highlightvar{c3}|})
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
[isinstance(@{|\highlightvar{n2}|}, pandas.DataFrame),
@{|\highlightvar{c1}|} in @{|\highlightvar{n2}|}.columns,
@{|\highlightvar{c2}|} in @{|\highlightvar{n2}|}.columns,
not @{|\highlightvar{n2}|}[@{|\highlightvar{c2}|}].isnull().any()]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
\\
\hline
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\scriptsize
Identical \\
Transformation \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
@{|\highlightast{expr}|: |\highlightvar{e1}|}= @{|\highlightast{expr}|: |\highlightvar{e2}|}.str.extract(@{|\highlightast{Const(str)}|: |\highlightvar{s1}|}, expand=False)
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15,escapeinside=||]{python}
@{|\highlightvar{e1}|}= @{|\highlightvar{e2}|}.str.extract(@{|\highlightvar{s1}|}, expand=False)
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
[type(@{|\highlightvar{e2}|}) == pandas.Series,
@{|\highlightvar{e2}|}.dtype == 'O' or pandas.api.types.is_string_dtype(@{|\highlightvar{e2}|}),
@{|\highlightvar{s1}|} == r'\((\d{4})\)']
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
\\
\hline
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\scriptsize
Over-Optimization\\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{v1}|}= @{|\highlightast{Name}|: |\highlightvar{v2}|}.shape[0]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15,escapeinside=||]{python}
@{|\highlightvar{v1}|}= @{|\highlightvar{v2}|}.__len__()
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
[hasattr(@{|\highlightvar{v2}|}, 'shape'),
isinstance(@{|\highlightvar{v2}|}.shape, tuple),
@{|\highlightvar{v2}|}.shape[0] == @{|\highlightvar{v2}|}.__len__()]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
\\
\hline
\rowcolor{lightgray!15}
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\scriptsize
Trivial \\
Preconditions \\
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
@{|\highlightast{Name}|: |\highlightvar{n1}|}= @{|\highlightast{Name}|: |\highlightvar{n2}|}.shape[0]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,bgcolor=lightgray!15,escapeinside=||]{python}
@{|\highlightvar{n1}|}= len(@{|\highlightvar{n2}|})
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
%\vspace{0pt}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere,escapeinside=||]{python}
[hasattr(@{|\highlightvar{n2}|}, 'shape'),
isinstance(@{|\highlightvar{n2}|}.shape, tuple),
len(@{|\highlightvar{n2}|}.shape) > 0,
len(@{|\highlightvar{n2}|}) == @{|\highlightvar{n2}|}.shape[0]]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
%\vspace{0pt}
$?$
\end{minipage}
\\
\hline
\end{tabular}
% %{2pt}
\label{tbl:plebian_rules}
\end{table*}
}

==> sections/tables/temp.tex <==
{
\footnotesize
\begin{table*}[t]
\caption{Plebian Categories}
\begin{tabular}
{p{0.10\textwidth}|p{0.18\textwidth}|p{0.18\textwidth}|p{0.28\textwidth}|p{0.04\textwidth}|p{0.04\textwidth}}
\toprule
%Row 1
\centering Category & \centering LHS & \centering RHS & \centering Preconditions & \centering Spd & \centering Freq\arraybackslash \\
\midrule
\begin{minipage}[t]{\linewidth}
\scriptsize
Expensive \\ Preconditions
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere]{python}
@{Name: n1} = @{Name: n2}.sample(@{Const(int): c1})
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere]{python}
@{n1} = @{n2}.loc[np.random.choice(@{n2}.index, size=@{c1}, replace=False)]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere]{python}
[isinstance(@{n2}, (pd.DataFrame, pd.Series)), @{c1} <= len(@{n2}), 
@{c1} >= 0, @{n2}.index.is_unique]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
$0.64\times$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
$?$
\end{minipage}
\\
\midrule
\begin{minipage}[t]{\linewidth}
\scriptsize
Datasize \\
Discrepensy
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize ,breaklines,breakanywhere]{python}
@{Name: n2}[ @{expr: e1} ][ @{Const(str): c1} ].unique()
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere]{python}
@{n1} = np.unique(@{n2}.loc[@{e1}, @{c1}].values)
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere]{python}
[isinstance(@{n2}, pandas.DataFrame),@{c1} in @{n2}.columns,
isinstance(@{e1}, (np.ndarray, pandas.Series, pandas.Index, list)) or
hasattr(@{e1}, '__array__')]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
$?\times$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
$?$
\end{minipage}
\\
\midrule
\begin{minipage}[t]{\linewidth}
\scriptsize
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize ,breaklines,breakanywhere]{python}
@{Name: n2}[ @{expr: e1} ][ @{Const(str): c1} ].unique()
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere]{python}
@{n1} = np.unique(@{n2}.loc[@{e1}, @{c1}].values)
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\begin{minted}[fontsize=\scriptsize,breaklines,breakanywhere]{python}
[isinstance(@{n2}, pandas.DataFrame),@{c1} in @{n2}.columns,
isinstance(@{e1}, (np.ndarray, pandas.Series, pandas.Index, list)) or
hasattr(@{e1}, '__array__')]
\end{minted}
\end{minipage}
&
\begin{minipage}[t]{\linewidth}
\centering
$?\times$
\end{minipage}
& 
\begin{minipage}[t]{\linewidth}
\centering
$?$
\end{minipage}
\\
\bottomrule
\end{tabular}
\label{tbl:plebian_rules}
\end{table*}
}
